Systematic event generator tuning for the LHC

In this article we describe Professor, a new program for tuning model parameters of Monte Carlo event generators to experimental data by parameterising the per-bin generator response to parameter variations and numerically optimising the parameterised behaviour. Simulated experimental analysis data is obtained using the Rivet analysis toolkit. This paper presents the Professor procedure and implementation, illustrated with the application of the method to tunes of the Pythia 6 event generator to data from the LEP/SLD and Tevatron experiments. These tunes are substantial improvements on existing standard choices, and are recommended as base tunes for LHC experiments, to be themselves systematically improved upon when early LHC data is available.

==> figs_ue_pT/Makefile <==
PLOTS = CDF_2000_S4155203_d01-x01-y01.pdf CDF_2001_S4751469_d03-x01-y01.pdf \
        CDF_2001_S4751469_d03-x01-y02.pdf CDF_2008_LEADINGJETS_d07-x01-y01.pdf \
        CDF_2008_LEADINGJETS_d09-x01-y01.pdf CDF_2008_NOTE_9337_d01-x01-y01.pdf \
        CDF_2008_NOTE_9351_d01-x01-y01.pdf CDF_2008_NOTE_9351_d07-x01-y01.pdf \
        CDF_2008_NOTE_9351_d19-x01-y01.pdf CDF_2008_NOTE_9351_d20-x01-y01.pdf
FULLRANGEPLOTS = CDF_2002_S4796047_d01-x01-y01.pdf CDF_2002_S4796047_d02-x01-y01.pdf

all: $(PLOTS) $(FULLRANGEPLOTS)

$(PLOTS): %.pdf: %.dat
	make-plots --cm --pdf $<

$(FULLRANGEPLOTS): %.pdf: %.dat
	make-plots --cm --pdf --full-range $<



==> figs_ue_q2/Makefile <==
PLOTS = CDF_2000_S4155203_d01-x01-y01.pdf CDF_2001_S4751469_d03-x01-y01.pdf \
        CDF_2001_S4751469_d03-x01-y02.pdf CDF_2008_LEADINGJETS_d07-x01-y01.pdf \
	CDF_2008_LEADINGJETS_d09-x01-y01.pdf CDF_2008_NOTE_9337_d01-x01-y01.pdf \
	CDF_2008_NOTE_9351_d01-x01-y01.pdf CDF_2008_NOTE_9351_d19-x01-y01.pdf

all: $(PLOTS)

$(PLOTS): %.pdf: %.dat
	make-plots --cm --pdf $<



==> profpythia6-preamble.tex <==
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{amsmath,amssymb,bm}
\usepackage{cite}
\usepackage{rotating}
\usepackage{relsize}
\usepackage{snapshot}
\usepackage{booktabs}
\usepackage[labelfont=bf]{caption}
%\usepackage{underscore}
\usepackage[italic]{hepparticles}
\usepackage{hepnames,hepunits}
\usepackage[small, nooneline]{subfigure}

%%% To work with JHEP.cls, (x)color.sty needs this work-around:
\usepackage{xcolor}
\makeatletter
\let\default@color\current@color
\makeatother

%%% I'm not sure if we really want to format URLs \smaller ...
\usepackage{url}
\makeatletter
\def\url@smallerstyle{%
  \@ifundefined{selectfont}{\def\UrlFont{\smaller}}{\def\UrlFont{\smaller}}}
\makeatother
\urlstyle{smaller}


\IfFileExists{microtype.sty}{%
  \RequirePackage{microtype}%
  %\RequirePackage[tracking=true]{microtype}%
  %\UseMicrotypeSet[tracking]{smallcaps}%
  %\SetTracking{encoding=*,shape=sc}{30}
}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\DeclareMathOperator{\det}{det}

\newcommand{\EqRef}[1]{equation~\eqref{#1}\xspace}
\newcommand{\SecRef}[1]{section~\ref{#1}\xspace}
\newcommand{\TabRef}[1]{Table~\ref{#1}\xspace}
\newcommand{\FigRef}[1]{Figure~\ref{#1}\xspace}
\newcommand{\TabsRef}[1]{Tables~\ref{#1}\xspace}
\newcommand{\FigsRef}[1]{Figures~\ref{#1}\xspace}

\newcommand{\p}{\ensuremath{\vec{p}}\xspace}
\newcommand{\pzero}{\ensuremath{\vec{p}_0}\xspace}
\newcommand{\pprime}{\ensuremath{\vec{p}^{\,\prime}}\xspace}
\newcommand{\N}[1]{\ensuremath{N^{\mspace{0.5mu}(\mspace{-0.5mu}#1)}}\xspace}
\newcommand{\Nn}[2]{\ensuremath{N_{\,#1}^{\mspace{0.5mu}(\mspace{-0.5mu}#2)}}\xspace}
\newcommand{\Nmin}[1]{\ensuremath{N_\text{min}^{\mspace{0.5mu}(\mspace{-0.5mu}#1)}}\xspace}
\newcommand{\Ndf}{\ensuremath{N_\text{df}}\xspace}
\newcommand{\Ptilde}{\ensuremath{\mathbf{\tilde{P}}}\xspace}
\newcommand{\ptilde}{\ensuremath{\tilde{p}}\xspace}
\newcommand{\vptilde}{\ensuremath{\vec{\tilde{p}}}\xspace}
\newcommand{\Ipseudo}{\ensuremath{\tilde{\mathcal{I}}}\xspace}
\newcommand{\DeltaOf}[1]{\ensuremath{\Delta\mspace{0.75mu}#1}\xspace}
\newcommand{\vcoeff}{\ensuremath{\vec{c}}\xspace}
\newcommand{\vcoeffb}{\ensuremath{\vec{c}^{(b)}}\xspace}
\newcommand{\coeffb}[1]{\ensuremath{c^{(b)}_{#1}}\xspace}
\newcommand{\vval}{\ensuremath{\vec{v}}\xspace}
\newcommand{\vvalb}{\ensuremath{\vec{v}^{(b)}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqNdf}{\ensuremath{\chi^2\!/\Ndf}\xspace}
\newcommand{\nCr}[2]{\ensuremath{\parenths{\colvec{#1 \\ #2}}}\xspace}
\newcommand{\wO}{\ensuremath{w_{\mathcal{O}}}\xspace}
\newcommand{\alphaS}{\ensuremath{\alpha_\text{s}}\xspace}
\newcommand{\pT}{\ensuremath{p_\perp}\xspace}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_\text{QCD}}\xspace}
\newcommand{\ofOrder}[1]{\ensuremath{\mathcal{O}(#1)}\xspace}
\newcommand{\kbd}[1]{{\smaller{\texttt{#1}}}}
\newcommand{\xparagraph}[1]{\par\vspace{2mm}\noindent\emph{#1}\quad}


\def\PARJ#1{\ensuremath{\text{PARJ(#1)}}}
\def\PARP#1{\ensuremath{\text{PARP(#1)}}}
\def\MSTJ#1{\ensuremath{\text{MSTJ(#1)}}}

%%% A very visible way of displaying TODOs:
\definecolor{todoboxcolor}{rgb}{1.0,0.6,0.6}
\newcommand{\TODO}[1]{\par\medskip \noindent%
\colorbox{todoboxcolor}{TODO: \parbox[t]{6.5cm}{#1}}%
\medskip\par}

\definecolor{todoneboxcolor}{rgb}{1.0,0.9,0.9}
\newcommand{\TODONE}[1]{\par\medskip \noindent%
\colorbox{todoneboxcolor}{TODONE?: \parbox[t]{6.5cm}{#1}}%
\medskip\par}


%%% Some names, to use a consistent spelling throughout the document:
\def\aleph{ALEPH\xspace}
\def\delphi{DELPHI\xspace}
\def\tasso{TASSO\xspace}
\def\opal{OPAL\xspace}
\def\lthree{L3\xspace}
\def\cdf{CDF\xspace}
\def\dzero{D\O\xspace}
\def\ATLAS{ATLAS\xspace}
\def\cms{CMS\xspace}

\def\lep{LEP\xspace}
\def\lepi{LEP~1\xspace}
\def\lhc{LHC\xspace}
\def\tevatron{Tevatron\xspace}
\def\rhic{RHIC\xspace}
\def\hera{HERA\xspace}
\def\sld{SLD\xspace}

\def\fnal{FNAL\xspace}
\def\cern{CERN\xspace}

\def\mcnet{MCnet\xspace}
\def\pdg{PDG\xspace}

\def\runi{Run-\textsmaller{I}\xspace}
\def\runii{Run-\textsmaller{II}\xspace}
\def\runiia{Run-\textsmaller{II}a\xspace}
\def\runiib{Run-\textsmaller{II}b\xspace}

\def\Cpp{C\raisebox{0.2ex}{\smaller++}\xspace}

\def\fortran{Fortran\xspace}
\def\pythia{Pythia\xspace}
\def\pythiasix{Pythia~6\xspace}
\def\pythiaeight{Pythia~8\xspace}
\def\herwig{Herwig\xspace}
\def\herwigsix{Herwig~6\xspace}
\def\herwigpp{Herwig\raisebox{0.1ex}{\smaller++}\xspace}
\def\sherpa{Sherpa\xspace}
\def\alpgen{AlpGen\xspace}
\def\charybdis{Charybdis\xspace}
\def\jimmy{Jimmy\xspace}
\def\rivet{Rivet\xspace}
\def\rivetgun{Rivetgun\xspace}
\def\professor{Professor\xspace}
\def\fastjet{FastJet\xspace}
\def\hepmc{HepMC\xspace}
\def\agile{AGILe\xspace}
\def\hztool{HZTool\xspace}
\def\numpy{NumPy\xspace}
\def\scipy{SciPy\xspace}
\def\minuit{Minuit\xspace}
\def\pyminuit{PyMinuit\xspace}
\def\python{Python\xspace}

\def\jade{Jade\xspace}
\def\durham{Durham\xspace}

\def\gof{GoF\xspace}

